Efficient Feature Interactions with Transformers: Improving User Spending Propensity Predictions in Gaming

Dream11 is a fantasy sports platform that allows users to create their own virtual teams for real-life sports events. We host multiple sports and matches for our 200M+ user base. In this RMG (real money gaming) setting, users pay an entry amount to participate in various contest products that we provide to users. In our current work, we discuss the problem of predicting the user's propensity to spend in a gaming round, so it can be utilized for various downstream applications. e.g. Upselling users by incentivizing them marginally as per their spending propensity, or personalizing the product listing based on the user's propensity to spend. We aim to model the spending propensity of each user based on past transaction data. In this paper, we benchmark tree-based and deep-learning models that show good results on structured data, and we propose a new architecture change that is specifically designed to capture the rich interactions among the input features. We show that our proposed architecture outperforms the existing models on the task of predicting the user's propensity to spend in a gaming round. Our new transformer model surpasses the state-of-the-art FT-Transformer, improving MAE by 2.5\% and MSE by 21.8\%.

==> text/why-deep-learning.tex <==
  
\subsection{Pretrained models for tabular data and fine-tuning for downstream use cases}
Building pre-trained models for text and image tasks and fine-tuning them for downstream tasks has been a common practice in deep learning. This was facilitated by the availability of large data like crawls of the web and large image datasets.
We dont have large publicly available tabular datasets like we have for text and image data. But, we can still use the pre-trained models for company-specific tabular data and fine-tune them for downstream tasks. i.e. we want to predict user churn, repeat purchase, fraud detection, user spends propensity and some dream11-specific use cases like user deposit amount prediction, user team withdrawal prediction etc. Although the problem statement is different but shares a lot of similarities in feature space. The current state is building models from scratch for each use case. While this is a good approach, it is not scalable as maintaining all these models and refreshing them with new data is a big task. 
The idea is to build a pre-trained model for tabular data and fine-tune it for downstream tasks. This will reduce the time to production and also reduce the maintenance cost.
It can be really useful for current use cases like churn prediction where they wanted to predict time-series of nth day churn. The current process is to build a model for each day. But if we have a pre-trained model for churn, we can fine-tune easily for each day. This will also help in new user churn prediction where you fine-tune the model on a small dataset of labeled data. This increases the velocity of releasing new models.



\subsection{Embedding Hub for downstream tasks}
We have seen the success of word embeddings in NLP tasks. We can use the same concept for tabular data. We can use the embeddings for tabular data to capture the complex patterns in the data.  
We can build a hub for tabular data embeddings and use them for downstream tasks. This will help us to build better models for tabular data and also reduce the time to production. The embeddings are not parametric as these can be trained in an unsupervised way and can be used for downstream tasks. These embeddings are rich sources of information just like word embeddings.[yC1YsBga] 
[Roman et al.2023](https://arxiv.org/abs/2206.15306) mentioned that neural models learn reusable features and are easily fine-tuned in new domains.  
Guang Liu et al.2022 also highlighted the importance of embeddings in tabular data. They showed that the embeddings can capture the complex patterns in the tabular data and can be used for downstream tasks.[^NBVRJlye]  

These embeddings are not vanilla embeddings. We usually train embeddings for deep-learning models. Trained embeddings are just task-specific. They are not contextualized. They are embeddings that are trained for a specific task. However, contextual embeddings are trained on a large dataset and can be used for multiple tasks.

To visualize, consider the image of trained contextual embeddings below. Two categorical features are highlighted —relationship (black) and marital status (blue). These features are related, so values of “Married”, “Husband” and “Wife” should be close to each other in the vector space even though they come from different variables.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/image.png}
    \caption{TabtransformerEmbeddings}
    \label{fig:enter-label}
\end{figure}


With trained contextual embeddings, we can indeed see that marital status of “Married” is closer to the relationship levels of “Husband” and “Wife”, whereas “non-married” categorical values from separate clusters to the right. This type of context makes these embeddings more useful and it would not have been possible using trained categorical embeddings.
This makes the case that embeddings are rich features and can be used for downstream tasks. This is not just true for categorical variables, but also for continuous variables.
[Yuri et al. 2022](https://arxiv.org/pdf/2203.05556.pdf) mentioned that embeddings for continuous variables significantly improve the performance of the model. 
We can also directly use these embeddings as features for traditional ML models even if somebody is not good with deep learning.
It would be nice to see the performance comparison of embeddings as features for GBDT models.  
Recently Uber talked about how they are using embeddings in their [use-cases](https://www.uber.com/en-IN/blog/innovative-recommendation-applications-using-two-tower-embeddings/). 
Another paper from Uber talking about next wave of building model where they are weighing on [embeddings](https://arxiv.org/pdf/2108.05053.pdf)
Uber calls them Two Tower embeddings and they are using them for many downstream use-cases eliminating the feature engineering.

Embeddings also serve use cases based on similarity measures i.e. if we want to get similar rounds, similar contests, and similar users. The current state relies on basic methods like similar CEA. Even if some use cases are using embeddings, they are not reusable as they are task-specific.  

The current state is that we do see interest from multiple internal teams to use embeddings, but current embeddings are parametric and task-dependent. This will help in building a hub for embeddings and can be used for downstream tasks. These reusable embeddings will also help in reducing the cost as we have multiple pipelines which run daily to compute features. 

Embeddings can be divided further to capture long-term interest and short-term interest. One is static and other is dynamic embeddings. This can be used for use-cases like user personalization where we want to capture the long-term and short-term interest of the user.

\subsection{Multi-Task Learning}
Multi-task learning involves training a model on multiple related tasks simultaneously. This technique can be useful in scenarios where the tasks share some common features or have related objectives. For example, a model can be trained on a dataset of customer purchase history and demographic data to predict customer churn and recommend new products. In this scenario, the model learns to capture the patterns that are common to both tasks, such as customer preferences and purchase behavior, while also learning to perform specific tasks.
This is not possible with traditional ML models as they were designed for single-task learning. But deep learning models can be trained on multiple tasks simultaneously. This can help in building better models for tabular data and also reduce the time to production.


\subsection{Semi-supervised and Self-supervised learning for tabular data}
This can come handy in use cases where we want to use machine learning quickly to our use case but we dont have any labeled or small-size labeled datasets. 
Use cases where getting labeled data is expensive and time-consuming. We can quickly get started using semi-supervised and self-supervised learning. i.e. When we wanted to build match center personalisation model, it was difficult to get labels as we needed to identify the new users contest joins at every minute in history. It was expensive to get the labels. Another example was when we needed to predict the real-time FPS prediction we did not have the label we wanted to predict and we had to modify the problem statement. There can be several other use cases where getting labeled data is difficult.
All these use cases can be solved using semi-supervised and self-supervised learning. 

